Recovery under Side Constraints

This paper addresses sparse signal reconstruction under various types of structural side constraints with applications in multi-antenna systems. Side constraints may result from prior information on the measurement system and the sparse signal structure. They may involve the structure of the sensing matrix, the structure of the non-zero support values, the temporal structure of the sparse representationvector, and the nonlinear measurement structure. First, we demonstrate how a priori information in form of structural side constraints influence recovery guarantees (null space properties) using L1-minimization. Furthermore, for constant modulus signals, signals with row-, block- and rank-sparsity, as well as non-circular signals, we illustrate how structural prior information can be used to devise efficient algorithms with improved recovery performance and reduced computational complexity. Finally, we address the measurement system design for linear and nonlinear measurements of sparse signals. Moreover, we discuss the linear mixing matrix design based on coherence minimization. Then we extend our focus to nonlinear measurement systems where we design parallel optimization algorithms to efficiently compute stationary points in the sparse phase retrieval problem with and without dictionary learning.

==> images/Cobras/texMacros.tex <==
% newcommands
\newcommand{\tj}{\text{\sf j}}
\newcommand{\tT}{\text{\sf T}}
\newcommand{\tH}{\text{\sf H}}
\newcommand{\tF}{\text{\sf F}}
\newcommand{\tfor}{\text{ for }}
\newcommand{\telse}{\text{ else }}
\newcommand{\tif}{\text{ if }}
\newcommand{\tst}{{\rm s.t.}}
\newcommand{\tsnr}{{\rm SNR}}
\newcommand{\tdB}{{\rm \,dB}}
\newcommand{\tE}{\ensuremath{\text{E}}}
\newcommand{\te}{\ensuremath{\text{e}}}
\renewcommand{\P}[1]{\ensuremath{\text{P}\left(#1\right)}}
\newcommand{\diag}{{\rm diag}}
\newcommand{\blkdiag}{\ensuremath{\text{blkdiag}}}
\renewcommand{\vec}{\ensuremath{{\rm vec}}}
\newcommand{\vecd}[1]{\ensuremath{\text{vecd}\left(#1\right)}}
\newcommand{\tr}{{\rm Tr}}
\newcommand{\rank}{{\rm rank}}
\newcommand{\real}[1]{\ensuremath{\text{Re}\left\{#1\right\}}}
\newcommand{\imag}[1]{\ensuremath{\text{Im}\left\{#1\right\}}}
% \newcommand{\supp}[1]{\ensuremath{\text{supp}\left\{#1\right\}}}
\newcommand{\supp}{\ensuremath{\mathcal{I}}}
\newcommand{\mb}[1]{\ensuremath{\mathit{\boldsymbol{#1}}}}
\newcommand{\bmtx}{\ensuremath{\begin{bmatrix}}}
\newcommand{\emtx}{\ensuremath{\end{bmatrix}}}
\newcommand{\mtx}[1]{\ensuremath{\begin{bmatrix} #1 \end{bmatrix}}}
\newcommand{\toep}{{\rm Toep}}
% \newcommand{\opt}[1]{\ensuremath{{#1}^{\star}}}
\newcommand{\opt}[1]{\ensuremath{\smash{\hat{#1}}}}
\newcommand{\true}[1]{\ensuremath{\smash{{#1}^\natural}}}
\newcommand{\sparse}[1]{\ensuremath{{#1}^\star}}
\newcommand{\pdMat}{\mathbb{D}_{+}}
\newcommand{\pdbMat}{\mathcal{B}_{+}}
\newcommand{\dMat}{\mathbb{D}}
\newcommand{\intSet}[1]{[#1]}
\def\myName{SPARROW}
\def\myNameB{Sparrow}
\newcommand{\mybar}{}
\def\coord{r}
\newcommand{\gray}[1]{\textcolor{lightgray}{#1}}

\DeclareMathOperator*{\argmin}{arg\,min}

% \renewcommand{\min}{\ensuremath{\textrm{min.}}}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proof}{Proof}


==> images/Cobras/tikzMacros.tex <==
% reduce linespacing in  legends
\pgfplotsset{every axis legend/.append style={row sep=-3pt, inner ysep=0pt, inner xsep=2pt}}

\def\tikzmark#1{\tikz[remember picture,overlay]\node[inner ysep=0pt,anchor=base](#1){\strut};}


% % for colorbars
% \pgfplotsset{colorbar/draw/.code={
%       \begin{axis}[
%         colormap/jet,
%         colorbar horizontal,
%         every colorbar,
% 		at={(0.5,1.1)},
% 		anchor=south,
% 		height=5pt,
% 		xticklabel pos=upper,
%         colorbar shift,
%         colorbar=false,
%       ]
%         \pgfkeysvalueof{/pgfplots/colorbar addplot}
%       \end{axis}
%     }]
% }

% alignment of tikzpictures in text
\tikzset{every picture/.append style={baseline=(current bounding box.north west)}}

% some parameters for the model images
\colorlet{cs0}{black!30!yellow}
\colorlet{cs1}{black!30!red}
\colorlet{cs2}{white!30!blue}
\colorlet{cs3}{black!25!green}
\colorlet{cs4}{black!20!orange}
\colorlet{cs5}{olive}
\colorlet{cs6}{brown}

% colormap for mtrix color random generator
\newcommand{\cla}{\pgfmathdeclarerandomlist{color}{{red}{red}{orange}};}
\newcommand{\clb}{\pgfmathdeclarerandomlist{color}{{blue}{blue}{teal}};}
\newcommand{\clc}{\pgfmathdeclarerandomlist{color}{{green!60!black}{green!80!black}{olive}};}
\newcommand{\cld}{\pgfmathdeclarerandomlist{color}{{brown!60!black}{brown}{gray}};}
\newcommand{\cle}{\pgfmathdeclarerandomlist{color}{{olive!60!black}{olive}{gray}};}
\newcommand{\clf}{\pgfmathdeclarerandomlist{color}{{violet}{purple}};}
\newcommand{\clg}{\pgfmathdeclarerandomlist{color}{{gray}{lightgray}};}
\newcommand{\clh}{\pgfmathdeclarerandomlist{color}{{black!25!yellow}{brown}};}

\newcommand{\bs}{3pt}

\tikzstyle{sensor}=[anchor=center,circle, fill=cs0, inner sep=0pt, minimum height=1.5mm]
\tikzstyle{sensor0}=[anchor=center,circle, fill=cs0, inner sep=0pt, minimum height=1.2mm]
\tikzstyle{sensor00}=[anchor=center,circle, fill=cs0, inner sep=0pt, minimum height=1.0mm]
\tikzstyle{source}=[anchor=center,fill=red, inner sep=0pt, minimum height=1.5mm, minimum width=1.5mm]
\tikzstyle{source0}=[anchor=center,fill=red, inner sep=0pt, minimum height=1.5mm, minimum width=1.5mm]
\tikzstyle{source00}=[anchor=center,fill=red, inner sep=0pt, minimum height=1.5mm, minimum width=1.2mm]
\tikzstyle{sensorBg}=[line width=3mm, line join=round, cap=round, fill=black!10, draw=black!10]
\tikzstyle{sensorBg0}=[line width=2.4mm, line join=round, cap=round, fill=black!10, draw=black!10]
\tikzstyle{sensorBg00}=[line width=1.4mm, line join=round, cap=round, fill=black!10, draw=black!10]
\tikzstyle{mybox} = [draw=blue!60, thick, rectangle, rounded corners, inner sep=10pt, inner ysep=15pt]
\tikzstyle{myboxsmall} = [draw=blue!60, thick, rectangle, rounded corners, inner sep=10pt, inner ysep=7.5pt]
\tikzstyle{fancytitle} =[fill=blue!60, text=white, rounded corners]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground} 

\def\NGrd{15}
\def\NSen{7}
\def\NSnp{4}
\def\dAng{12}
\def\angA{132}
\def\angB{96}
\def\angC{36}
\def\dA{3}
\def\dB{5}
\def\dC{10}
\def\seedA{107}
\def\seedB{198}
\def\cRange{60}

% seed for random number generator
\def\seedA{20}
\def\seedB{500}

\def\doaA{4}
\def\doaB{7}
\def\doaC{13}

% full matrix
\newcommand{\drawMtx}[5]{
	\begin{tikzpicture}[baseline=(current bounding box.south)]
		#4
		\pgfmathsetseed{#5}
		\foreach \x in {1,...,#2}{
		\foreach \y in {1,...,#1}{
			\pgfmathrandomitem{\c}{color};
			\pgfmathrandominteger{\r}{75}{100};
			\fill[\c!\r] (\x*#3, \y*#3) rectangle +(#3,#3);
		}
		}
	\end{tikzpicture}
}

% full matrix
\newcommand{\drawMtxH}[5]{
	\begin{tikzpicture}[baseline=(current bounding box.south)]
		#4
		\pgfmathsetseed{#5}
		\foreach \x in {1,...,#2}{
		\foreach \y in {1,...,#1}{
			\pgfmathrandomitem{\c}{color};
			\pgfmathrandominteger{\r}{75}{100};
			\fill[\c!\r] (\x*#3, -\y*#3) rectangle +(#3,#3);
			\fill[\c!\r] (\y*#3, -\x*#3) rectangle +(#3,#3);
		}
		}
	\end{tikzpicture}
}

% full matrix
\newcommand{\drawMtxB}[4]{
	\begin{tikzpicture}
		\foreach \x in {1,...,#3}{
		\foreach \y in {1,...,#2}{			
			\pgfmathrandominteger{\r}{50}{100};
			\fill[#1!\r] (\x*#4, \y*#4) rectangle +(#4,#4);
		}
		}
	\end{tikzpicture}
}

\newcommand{\grayVb}{  
	\begin{tikzpicture}[baseline=-1.5*\bs]
		\fill[red] (0pt, 0 pt) rectangle +(\bs,\bs);
		\clb;
		\foreach \y in {1}{
			\pgfmathrandomitem{\c}{color};
			\pgfmathrandominteger{\r}{75}{100}
			\fill[\c!\r] (0pt, -\y*\bs) rectangle +(\bs,\bs);
		}
		\clc;
		\foreach \y in {2}{
			\pgfmathrandomitem{\c}{color};
			\pgfmathrandominteger{\r}{75}{100}
			\fill[\c!\r] (0pt, -\y*\bs) rectangle +(\bs,\bs);
		}
	\end{tikzpicture}
}

\newcommand{\grayVc}{  
	\begin{tikzpicture}[baseline=-\bs+0.5pt]
		\cld
		\foreach \x in {0,1,...,5}{
			\pgfmathrandomitem{\c}{color};			
			\pgfmathrandominteger{\r}{80}{100}
			\fill[\c!\r] (\x*\bs, 0pt) rectangle +(\bs,\bs);
		}
	\end{tikzpicture}
}



==> non_circular.tex <==
%\section{Recovery algorithms under different side constraints for the linear measurement model}

%\subsection{Non-Circularity}

\marginpar{Marc: Can we use less ``we'' here? I think this should not
directly read as if it is a report, but also to inspire readers to read the
cited papers.}
\marginpar{Marius: Yes we can. Fixed!}

Recently, three different sparse recovery strategies have been proposed~\cite{SRH:16,SSPH:16,SRSHP:16} for exploiting the strict non-circularity property  of the impinging signals~\cite{Steinwandt2016nccrb,Steinwandt2017smoo}, i.e., the received complex symbols result from real-valued constellations 
rotated by an arbitrary phase $\phi$. As the rotation phase $\phi$ is usually unknown, the estimation 
problem becomes a two-dimensional (2-D) sparse recovery problem, which requires estimating the support 
in the spatial domain as well as in the rotation phase domain.

In~\cite{SRH:16}, a combined 2-D finite dictionary was introduced for both dimensions
and solve the resulting 2-D sparse recovery problem by $\ell_{2,1}$-mixed norm relaxation using multiple measurement vectors (MMV). Thereby,
the known benefits associated with strictly non-circular (NC) sources~\cite{Steinwandt2016nccrb,Steinwandt2017smoo}, e.g., an improved estimation accuracy and a doubling of the number of resolvable 
signals, can also be achieved via sparse recovery. In order to handle the resulting 2-D off-grid problem, an off-grid estimation procedure was introduced by means of local interpolation.

In~\cite{SSPH:16} addresses the prohibitive computational complexity required for
solving the 2-D mixed-norm problem as a result of sampling both dimensions, which significantly increases
the problem size. Thus in~\cite{SSPH:16}, a sparse optimization framework was proposed based on nuclear
norm (rank) minimization after lifting the original optimization problem to a semidefinite
programming (SDP) problem in a higher-dimensional
space. To this end, the 2-D estimation problem is reduced to a 1-D estimation problem only in the sampled
spatial domain, which automatically provides grid-less estimates of the rotation phases. As a result, the
proposed method requires a significantly lower computational complexity while providing the same performance
benefits. Additionally, an off-grid estimator for the spatial domain has been proposed.

In~\cite{SRSHP:16}, a grid-less sparse recovery algorithm for NC signals has been proposed
based on atomic norm minimization (ANM). After the NC preprocessing step, the ANM-equivalent SDP problem
provides a solution matrix with a two-level Hermitian Toeplitz structure. It was shown 
that by using the multidimensional generalization of the Vandermonde decomposition, the desired direction
estimates can be uniquely extracted from the two-level Hermitian Toeplitz matrix via NC Standard ESPRIT or NC Unitary ESPRIT~\cite{HR_icassp:04}
 in closed-form. 
 Due to the exploitation of the NC signal structure, the proposed NC ANM procedure provides a superior estimation accuracy  as compared to the original methods for arbitrary signals. In this case, the number of estimated sources can exceed the number of sensors in the array.
 
 


==> util_def.tex <==


%---- color things

\definecolor{light-gray}{gray}{0.65}
\def\blue{\color{blue}}
\def\red{\color{red}}
%%%%%%%%%

\newcommand{\setliteblue}{\color[rgb]{0,0.4,.6}}
\newcommand{\highlite}{\bf\color{blue}}
%\newcommand{\note}[1]{{\color{red} #1}}


%----notation abbreviations
\newcommand{\vect}[1]{\ensuremath{\mathbf{#1}}}
\newcommand\ba{\ensuremath{\mathbf{a}}}
\newcommand\bb{\ensuremath{\mathbf{b}}}
\newcommand\bc{\ensuremath{\mathbf{c}}}
\newcommand\bd{\ensuremath{\mathbf{d}}}
\newcommand\be{\ensuremath{\mathbf{e}}}
% cannot define \bf
\newcommand\bg{\ensuremath{\mathbf{g}}}
\newcommand\bh{\ensuremath{\mathbf{h}}}
\newcommand\bn{\ensuremath{\mathbf{n}}}
\newcommand\bq{\ensuremath{\mathbf{q}}}
\newcommand\br{\ensuremath{\mathbf{r}}}
\newcommand\bs{\ensuremath{\mathbf{s}}}
\newcommand\bu{\ensuremath{\mathbf{u}}}
\newcommand\bv{\ensuremath{\mathbf{v}}}
\newcommand\bw{\ensuremath{\mathbf{w}}}
\newcommand\bx{\ensuremath{\mathbf{x}}}
\newcommand\by{\ensuremath{\mathbf{y}}}
\newcommand\bz{\ensuremath{\mathbf{z}}}

\newcommand\bA{\ensuremath{\mathbf{A}}}
\newcommand\bB{\ensuremath{\mathbf{B}}}
\newcommand\bC{\ensuremath{\mathbf{C}}}
\newcommand\bD{\ensuremath{\mathbf{D}}}
\newcommand\bE{\ensuremath{\mathbf{E}}}
\newcommand\bF{\ensuremath{\mathbf{F}}}
\newcommand\bG{\ensuremath{\mathbf{G}}}
\newcommand\bH{\ensuremath{\mathbf{H}}}
\newcommand\bI{\ensuremath{\mathbf{I}}}
\newcommand\bL{\ensuremath{\mathbf{L}}}
\newcommand\bM{\ensuremath{\mathbf{M}}}
\newcommand\bP{\ensuremath{\mathbf{P}}}
\newcommand\bQ{\ensuremath{\mathbf{Q}}}
\newcommand\bR{\ensuremath{\mathbf{R}}}
\newcommand\bS{\ensuremath{\mathbf{S}}}
\newcommand\bT{\ensuremath{\mathbf{T}}}
\newcommand\bU{\ensuremath{\mathbf{U}}}
\newcommand\bV{\ensuremath{\mathbf{V}}}
\newcommand\bW{\ensuremath{\mathbf{W}}}
\newcommand\bX{\ensuremath{\mathbf{X}}}
\newcommand\bY{\ensuremath{\mathbf{Y}}}
\newcommand\bZ{\ensuremath{\mathbf{Z}}}

\newcommand\bzero{\ensuremath{\mathbf{0}}}
\newcommand\bone{\ensuremath{\mathbf{1}}}

%\newcommand\lam{\ensuremath{{\lambda}}}
\newcommand\balpha{\ensuremath{\boldsymbol{\alpha}}}
\newcommand\bbeta{\ensuremath{\boldsymbol{\beta}}}
\newcommand\bmu{\ensuremath{\boldsymbol{\mu}}}
\newcommand\bnu{\ensuremath{\boldsymbol{\nu}}}
\newcommand\bphi{\ensuremath{\boldsymbol{\phi}}}
\newcommand\bdelta{\ensuremath{\boldsymbol{\delta}}}

\newcommand\bDelta{\ensuremath{\boldsymbol{\Delta}}}
\newcommand\bTheta{\ensuremath{\boldsymbol{\Theta}}}
\newcommand\bLambda{\ensuremath{\boldsymbol{\Lambda}}}
\newcommand\bSigma{\ensuremath{\boldsymbol{\Sigma}}}
\newcommand\bPhi{\ensuremath{\boldsymbol{\Phi}}}
\newcommand\bOmega{\ensuremath{\boldsymbol{\Omega}}}

\newcommand{\Rbb}{\ensuremath{\mathbb{R}}}
\newcommand{\Cbb}{\ensuremath{\mathbb{C}}}
\newcommand{\Sbb}{\ensuremath{\mathbb{S}}}
\newcommand{\Hbb}{\ensuremath{\mathbb{H}}}
\newcommand{\Kbb}{\ensuremath{\mathbb{K}}}

\newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\opr}[1]{\ensuremath{\mathcal{#1}}}

%\newcommand\jj{\ensuremath{\boldsymbol{j}}}
%\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\Arg}{Arg}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Diag}{Diag}
\DeclareMathOperator{\tr}{tr}
\newcommand\nnz{\ensuremath{{\rm nnz}}}
\newcommand\sspan{\ensuremath{{\rm span}}}

\newcommand{\bigO}{\mathcal{O}}

\newcommand{\norm}[1]{\lVert {#1} \rVert}
\newcommand{\Norm}[1]{\left\lVert {#1} \right\rVert}
\newcommand{\abs}[1]{\lvert {#1} \rvert}
\newcommand{\Abs}[1]{\left\lvert {#1} \right\rvert}
\newcommand{\ceil}[1]{\lceil{#1}\rceil}
\newcommand{\floor}[1]{\lfloor{#1}\rfloor}

\newcommand{\tT}{\ensuremath{{\text{T}}}}
\newcommand{\tH}{\ensuremath{{\text{H}}}}
\newcommand{\tF}{\ensuremath{\text{F}}}
\newcommand{\st}{\text{s.t.}}
\newcommand{\suchthat}{\,:\,}
\newcommand{\NP}{\textsf{NP}}
\renewcommand{\P}{\textsf{P}}
\renewcommand{\vec}{\ensuremath{\operatorname{vec}}}

